TART: A plug-and-play Transformer module for task-agnostic reasoning

Large language models (LLMs) exhibit in-context learning abilities which enable the same model to perform several tasks without any task-specific training. In contrast, traditional adaptation approaches, such as fine-tuning, modify the underlying models for each specific task. In-context learning, however, consistently underperforms task-specific tuning approaches even when presented with the same examples. While most existing approaches (e.g., prompt engineering) focus on the LLM's learned representations to patch this performance gap, our analysis actually reveal that LLM representations contain sufficient information to make good predictions. As such, we focus on the LLM's reasoning abilities and demonstrate that this performance gap exists due to their inability to perform simple probabilistic reasoning tasks. This raises an intriguing question: Are LLMs actually capable of learning how to reason in a task-agnostic manner? We answer this in the affirmative and propose TART which generically improves an LLM's reasoning abilities using a synthetically trained Transformer-based reasoning module. TART trains this reasoning module in a task-agnostic manner using only synthetic logistic regression tasks and composes it with an arbitrary real-world pre-trained model without any additional training. With a single inference module, TART improves performance across different model families (GPT-Neo, Pythia, BLOOM), model sizes (100M - 6B), tasks (14 NLP binary classification tasks), and even across different modalities (audio and vision). Additionally, on the RAFT Benchmark, TART improves GPT-Neo (125M)'s performance such that it outperforms BLOOM (176B), and is within 4% of GPT-3 (175B). Our code and models are available at https://github.com/HazyResearch/TART .

==> app/hyena.tex <==
\section{Generalization of TART beyond Transformer architecture}\label{app:sec-2}
In this section, we demonstrate that non-transformer based sequence architectures~\citep{poli2023hyena} can be used for the TART reasoning module. Concretely, we demonstrate that a Hyena reasoning module~\citep{poli2023hyena}, trained on the same synthetic logistic regression tasks, can also be composed with LLMs to improve in-context learning performance.

\subsection{Set-up and Training Details}
We train a model with sequence length 
\subsection{Results}

==> bak/abs_v1.tex <==
\begin{comment}
% This is version 1
Large language models (LLMs) exhibit in-context ability, a task-agnostic form of learning, which enables one to use the same model for several different downstream tasks in a few-shot manner.
%In-context ability of LLMs has enabled task-agnostic learning, where the same model can be used for several different downstream tasks. 
However, even when presented with the same data, a big performance gap exists between in-context learning and task-specific methods (for example, fine-tuning or training adapter heads). In this work, we study why such a performance gap exists between in-context learning and the task-specific training methods. We show that while the language models learn good representations for the task during the autoregressive pre-training, their performance is bottlenecked by their ability to reason over these representations. 

Based on these insights, we propose a new method, \alg, which improves this generic reasoning deficiency of LLMs in a task-agnostic manner. \alg grafts a pre-trained LLM with a general-purpose inference module, which is trained entirely on synthetically generated probabilistic inference data. We show that a single inference module works across different model families (GPT-Neo, Pythia, Bloom), different model sizes (100M, 500M, 1B, 2B), different tasks (14 different NLP tasks), as well as across modalities (speech and vision). In addition to being \emph{task, model, and domain agnostic}, \alg overcomes the context-window bottleneck of in-context learning and is \emph{data-scalable} -- it can work with up to 20x the number of datapoints as compared to vanilla in-context learning. In terms of \emph{performance quality}, \alg improves upon in-context learning on XX out of the 14 tasks, on average giving an accuracy gain of YY pts, and is within XX\% of task-specific approaches on YY tasks.
\end{comment}
% Version 2
\kbcomm{Large language models (LLMs) exhibit in-context ability that enables the same model to perform several downstream tasks without any retraining.} Large language models (LLMs) exhibit in-context ability, a task-agnostic form of learning that enables the same model to perform several downstream tasks. In contrast, traditional task adaptation approaches (such as fine-tuning) modify the underlying models for \emph{each} specific task.
While in-context learning is task-agnostic, it 1) is not data-scalable due to its context window bottleneck, limiting its effective use of examples, and 2) has lower performance quality, when compared with fine-tuning, even when presented with the same examples. We investigate why this surprising quality gap exists – is it because of insufficient information in the learnt representations or because the LLMs are unable to perform reasoning over them. We experimentally observe that task-specific adapters trained on these LLM representations can recover up to 90\% of the performance gap, and it is therefore their inability to reason which bottlenecks performance.


Based on these insights, we propose \alg which improves this generic reasoning deficiency of LLMs. \alg trains an independent transformer-based inference module using only synthetically generated logistic regression tasks. It then fuses this inference module with a pre-trained LLM to improve upon its task-agnostic learning abilities. 
%
With a single independently trained inference module, \alg improves the base model performance across different model families (GPT-Neo, Pythia, BLOOM), different model sizes (100M - 2B), different tasks (14 NLP classification tasks), and works even across modalities (speech and vision).
%
%\alg improves the base model performance across different model families (GPT-Neo, Pythia, Bloom), different model sizes (100M, 500M, 1B, 2B), different tasks (14 NLP classification tasks), and works even across modalities (speech and vision) using the same independently trained inference module. 
\alg is data-scalable and works with up to 20x the number of examples as compared to vanilla in-context learning. %, by using only 2 tokens to represent each example. 
In terms of performance quality, \alg improves upon in-context learning on XX out of the 14 tasks, on average giving an accuracy gain of YY pts, and is within XX\% of task-specific approaches on YY tasks.

\kbcomm{Alternate is to remove: "\alg trains an independent transformer-based inference module using only synthetically generated logistic regression tasks. \alg then fuses this inference module with a pre-trained LLM model to improve upon its task-agnostic learning abilities" from the second paragraph.}

==> bak/intro.tex <==
\section{Introduction}\label{sec:intro}
Large language models (LLMs) like GPT-Neo~\citep{gpt-neo}, Pythia, and BLOOM show in-context learning capabilities which enables them to perform a task given only a few examples, without updating the model parameters. This task-agnostic capability allows for a single model to be applied to a wide range of tasks. In contrast, traditional task adaptation approaches, such as fine-tuning and adapters, update the model parameters for each specific task.
% have enabled task-agnostic learning in the form of in-context learning. This in-context learning ability enables models to perform a task using only a few demonstrations , without being explicitly trained for it and allows one to use the same model for multiple tasks. 


%Foundation models like GPT, Pythia, and Bloom have enabled task-agnostic learning in the form of in-context learning. This in-context ability enables models to perform a task from a few demonstrations provided by the user,  without being explicitly trained for it and allows the same model to be used for multiple downstream applications.\ancomm{maybe line break here}This task-agnostic property of in-context learning is in stark contrast \kbcomm{stark is to extreme} to more traditional learning approaches, such as fine-tuning and adaptor heads, which adapt a foundation model to a specific task. 

Typically, in-context learning is used in the few-shot regime since the number of examples that can be used is often bottlenecked by the LLM's context window. For instance, the GPT-Neo class of models have a context window of 2048 tokens, which can accommodate at most 10 examples, assuming each example requires around 200 tokens. Most existing works have attributed the performance gap between in-context learning and task-specific fine-tuning methods to this limited context window~\citep{kocon2023chatgpt}. 

However, this performance gap between in-context learning and fine-tuning approaches exists \emph{even} when presented with the same task examples (Figure~\ref{fig:macro}). %Despite being presented with the same information, there is an asymmetry in the performance across these methods. 
We would like to understand whether this gap is a generic limitation of task-agnostic methods for adaptation or is it specific to in-context learning? More precisely, can we design adaptation approaches which satisfy the following desiderata:
\begin{itemize}\vspace{-2mm}
    \item \emph{Task-agnostic}: Same model generalizes across several different tasks.\vspace{-1mm}
    \item \emph{Quality}: Achieves accuracy competitive with task-specific methods across these different tasks.\vspace{-1mm}
    \item \emph{Data-scalable}: The method can scale with number of task-specific examples available.
    %\item Model preservation: minimal changes to the base model and its representations \kbcomm{Change last one to Scales with examples }
\end{itemize}
We investigate why this quality gap exists between in-context learning and task-specific adaptation methods: is it because the learnt representations\footnote{We take the final layer embeddings of these language models as their learnt representations.} do not contain sufficient information or because the LLMs are unable to perform reasoning over these representations? 
We define the representation quality to be  insufficient if no classifier trained on these representations is able to perform the task well. Otherwise, we say that the representation have the required task-specific information and the reasoning capability is main bottleneck. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/table-algs-obj.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig-algs-change.png}
    \end{subfigure}
    \caption{\kbcomm{add caption}}
    \label{fig:algs}
\end{figure}

We explore this hypothesis experimentally in Section~\ref{sec:strats} by decomposing the performance gap into a reasoning and a representation gap. By observing both these quantities across a variety of LLM classes (GPT-Neo, Pythia, BLOOM) and a suite of binary classification tasks, we conclude that LLMs possess good representations, and the majority of the quality gap (up to 79\%) can be attributed to its reasoning ability (see Figure~\ref{fig:rep-reas}). Furthermore, we find that task adaptive methods (fine-tuning and adapter heads) improve the base model on both these axes, but majorly improve the task-specific reasoning ability which accounts for 72\% of the gained performance on the task.

% \begin{equation}
% \gapicl = \gaprep + \gapres\;,
% \end{equation}
% where $\gapicl$ represents the accuracy gap of in-context learning with respect to task-specific fine-tuning, $\gaprep$ represents the gap attributed to representation deficiency, and 

% In section XX, we study this hypothesis in detail and observe that for a large class of models (neo, pythia, bloom) foundation models are good at learning representations, but they lack good reasoning ability when evaluated via in-context learning. Furthermore, task adaptive methods (fine-tuning and adapter heads) improve the base model on both these axes, but majorly align (representation/reasoning) ability with the task accounting for almost yy\% of the gained performance on the task.


%\kbcomm{add 2 lines on limited number of examples for in-context learning, conventional wisdom on this being responsible for lower performance than fine tuning.}

%\kbcomm{reword this -- big gap in performance even when presented with the same training examples.} While in-context learning and traditional fine-tuning approaches, in principle, have access to the same examples from the dataset, there is a big gap in their relative performance. For instance, XX tasks, gpt-3 in-context performance is YY\% away from the SoTA task specific fine tuning (cite jack of all trades paper). Despite the symmetric information, we do not understand why this asymmetry in performance exists. Is this a fundamental limitation \kbcomm{maybe generic deficiency?}\ancomm{CDS says this wording sets up a theorem vs. what we say below} of task-agnostic methods for adaptation or is this specific to in-context learning? 

% More precisely, we would like a method for task adaptation which satisfies
% \begin{itemize}\vspace{-1.5mm}
%     \item Task-agnostic: same model works across many different tasks
%     \item Quality: achieves good accuracy across tasks
%     \item Model preservation: minimal changes to the base model and its representations \kbcomm{Change last one to Scales with examples }
% \end{itemize}
%\kbcomm{In this paper we consider two hypotheses why this gap might exist - representation or reasoning insufficiency?}
%The lack of performance quality for in-context learning can be attributed to one of two causes: either the task related representations that they are learning are insufficient or that they are limited by the ability to reason over those representations. In section XX, we study this hypothesis in detail and observe that for a large class of models (neo, pythia, bloom) foundation models are good at learning representations, but they lack good reasoning ability when evaluated via in-context learning. Furthermore, task adaptive methods (fine-tuning and adapter heads) improve the base model on both these axes, but majorly align (representation/reasoning) ability with the task accounting for almost yy\% of the gained performance on the task.

%\kbcomm{Explain these hypotheses and what these mean. The second paragraph will explain findings.}

These findings raise an intriguing question: Could it be that task-agnostic reasoning is beyond the capabilities of large language models? While the persistent quality gap between in-context learning and fine-tuning suggests this might be a generic limitation, we argue that the converse is in fact true. As a proof of concept, we propose \alg (see Figure~\ref{fig:main}) which improves this reasoning deficiency in a completely task-agnostic manner. 

\alg trains a transformer-based inference module using only synthetically generated logistic regression tasks, independent of the underlying task or the base language model. Surprisingly, this inference module can be composed \emph{without any additional training} with the embeddings of any LLM to improve upon its reasoning abilities. \alg demonstrates how we can compose, or \emph{graft}, two different transformer models - an LLM trained autoregressively on language data (representation learner) and an inference module trained entirely on synthetic data (reasoning ability). 
%\kbcomm{Say that it works, closes the gap, make it more specific, making a lot of points, make sure to unpack them here.} 
Notably, our method satisfies the desired objectives: 
\begin{itemize}\vspace{-2mm}
    \item \emph{Task agnostic}: \alg's inference module is only trained once using synthetic data.\vspace{-1mm}
    \item \emph{Quality}: Outperforms base LLM on all tasks and closes gap to task specific fine tuning methods.\vspace{-1mm}
    \item \emph{Data-scalable}: Can accommodate 10x more examples than in-context learning.\vspace{-1mm}
\end{itemize}
%
% with two different abilities - representation learning (from base backbone) and reasoning ability (from completely synthetic data).
% \kbcomm{LLM trained autoregressively on language data, inference module trained on synthetic data attempts almost closes the gap to fine-tuning.}
%\kbcomm{Bias-variance tradeoff error of NN into two components understand why a model performs worse -- bias vs variance error decomposition - maybe after neurips}
%\kbcomm{CR it is task agnostic, model agnostic, domain agnostic}
%\kbcomm{CR whats our view on baselines? - Can teach the model using synthetic data, but not scalable, and does not have good enough quality. why is this interesting to us? Adapter thing works across domains, models, Shows that this reasoning ability is not picked up from data}
\alg is task-agnostic, in the same way as in-context learning, and allows the same model to be used across different tasks. Using a single inference module trained on synthetic data, we demonstrate that \alg generalizes across three different model families (GPT-Neo, Pythia, Bloom) over 14 different NLP binary classification tasks (Figure~\ref{fig:macro}). Not only does this inference module work across different model families and tasks, it also generalizes across different domains---we show how the inference module, with the exact same weights, that was used for the NLP tasks, can be composed with vision and speech based foundation models ( Figure~\ref{fig:modalities}). Thus, the inference module is \emph{task, model, and domain agnostic}. 

In terms of quality, we show that \alg's performance is \red{XX} points better than in-context learning across tasks and is within \red{YY} points of task-specific fine-tuning and adapter head baselines across a suite of NLP tasks. On the RAFT subset of HELM evaluations, we show that the GPT-Neo (125M) model, when composed with \alg's inference module, can outperform OPT (175B) and Bloom (176B) models, and is within $4\%$ points of the GPT-3 (175B) model. 
%Furthermore, while each individual fine-tuning run takes about XX mins to train (in addition to the hyperparameter tuning), our inference module is extremely cheap to train (requires only 20 mins to train) and is robust to hyperparameter tuning. 
%Foundation models have enabled task-agnostic learning. This is in contrast to traditional ML wherein one adapts models to their tasks by precisely defining the task, curating data for the task in question and then training a model. Foundation models, on the other hand, allows the same model to be used for multiple different downstream applications.

\alg is data-scalable and overcomes the limited context length bottleneck of in-context learning. While each example spans across multiple tokens in a language model, often spanning hundreds of tokens, \alg's reasoning module encodes each example using only two tokens -- one for the context and the other for the label. %This allows us to use LLM embeddings and expand the number of examples that can be used at inference much beyond what in-context learning could allow. 
Figure~\ref{fig:} shows that this data-scalability can lead to performance improvements of up to $10\%$ points on long-context benchmarks.

%Foundation models like GPT-neo, Pythia, and Bloom have shown in-context ability -- the models learnt to perform a task from a few demonstrations provided by the user,  without being explicitly trained for it. The most interesting bit is that it allows users to use them for a variety of different tasks (task-agnostic) in a few-shot manner, without any training at inference time (model preservation).

%However, in terms of performance, these models are still not competitive with those adapted to the task. \ancomm{bring up challenges with context length}. For instance, XX tasks, gpt-3 in-context performance is YY\% away from the SoTA task specific fine tuning (cite jack of all trades paper). Different ways of adapting include fine tuning, partial fine tuning, and training task-specific adaptor heads. \ancomm{be less rushed here} While these methods have good performance, they are not task-agnostic. Moreover, they often change the model parameters significantly. Additionally, a major disadvantage of these task-adaptive methods is they get more expensive with scale (model parameters). \ancomm{introduce tension for why its counterintuitive that the ICL is worse thant SGD} 

%Key desiderata that we would therefore like a method to exhibit:

%Question we consider in our work: Can we design task-agnostic methods that require no training at inference time and perform as well as task-specific methods? 

%Our key insight is that while foundation models are good at learning representations, they lack good reasoning ability when evaluated via in-context learning. In exploring the differences between FT and ICL, we observe that task adaptation is dependent on two factors: representation quality and the ability to reason over those representations. In section XX, we study this hypothesis in detail and observe that for a large class of models (neo, pythia) task adaptive training methods improves the base model on both these axes, but majorly align (representation/reasoning) ability with the task accounting for almost yy\% of the gained performance on the task. 

% Based on this study, we propose a new method \alg(see figure 1), which uses the model embeddings in combination with a general-purpose probabilistic reasoning module to solve classification tasks. Key insight is one can use only synthetically generated Gaussian data to train this reasoning module, independent of the base model. Important aspects of the model are:
% \begin{itemize}
%     \item Task agnostic - is only trained once using synthetic data
%     \item Quality - for xx tasks, outperforms base model, closes gap to task adaptive fine tuned method.
%     \item Model preservation - requires no updates to the base model at inference time for learning task
% \end{itemize}
% \alg is completely plug and play module and demonstrates how we can graft transformer modules with two different abilities - representation learning (from base backbone) and reasoning ability (from completely synthetic data).
% From an empirical perspective, we extensively evaluate \alg across three different model families (Neo, Pythia, Bloom) over 14 different NLP binary classification tasks. We show that \alg's performance is XX points better than in-context learning across tasks and is within YY points of task-specific fine-tuning and adapter head baselines. Furthermore, while each individual fine-tuning run takes about XX mins to train (in addition to the hyperparameter tuning), our inference module is extremely cheap to train (requires only 20 mins to train) and is robust to hyperparameter tuning. Additionally, we show that the same reasoning module can also generalize across domains – for vision, with ViT embeddings achieves performance comparable to state of the art methods, and for speech, when combined with Whisper embeddings performs well. Thus, the inference module is task, model and domain agnostic. 


%demonstrate that \alg’s performance is within XX points of fine-tuning works across yy different NLP classification tasks for 3 different families of model classes. The inference module is cheap to train (requires only 20 mins to train)\kbcomm{add reasoning why it is interesting.}. Additionally, we show that the same reasoning module can also generalize across domains – for vision, with ViT embeddings achieves performance comparable to state of the art methods, and for speech, when combined with Whisper embeddings performs well. Thus, the inference module is task, model and domain agnostic. 

From a theoretical standpoint, we show that the generalization abilities of \alg depend mainly on the distribution shift between the natural text embedding distribution and the synthetic distribution, measured in terms of the Wasserstein-1 metric (Theorem~\ref{thm:gen}).
%We exhibit that this distance measure , is actually predictive of the performance gap of \alg from the fine tuned baselines with a correlation of xx (see Section xx).

%\ancomm{in this paper we do the following or we study we propose}
To summarize, our main contributions are as follows:
\begin{itemize}\vspace{-2mm}
\item Study why in-context learning does not perform as well as task-specific fine tuning despite having access to same information, via a representation-reasoning decomposition.\vspace{-1mm}
\item Propose a new task-agnostic method, \alg, which bridges the performance gap to task-specific methods and is trained using only synthetic data.\vspace{-1mm}
\item Empirically demonstrate that \alg works across different NLP tasks for a wide range of model families. The same inference module generalizes to vision and speech domains as well.
%\item Theoretically, we study the generalization properties of \alg and show that those are governed by the Wasserstein distance between the embedding and the synthetic distribution.\kbcomm{remove this point from the list}
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.05\textwidth]{figures/fig-main.png}
    \caption{\kbcomm{add caption}}
    \label{fig:main}
\end{figure}

==> bak/rel.tex <==
\section{Related work}
\label{sec:rel-work}

% \begin{wrapfigure}{r}{0.40\textwidth}
%    \centering\hspace*{-4ex}
%    \vspace{-15mm}
% %  \captionsetup{font=small}
% % \begin{tabular}{cc}
% %   \includegraphics[scale= 0.20, trim = 0 0 0 4, clip]{figures/S1_t2.png}&
% %   \includegraphics[scale= 0.20, trim = 0 0 0 4, clip]{figures/S2_t1.png}\\
% % (a)&(b)
% % \end{tabular}

% \includegraphics[width=0.4\textwidth, trim = 2 0 0 2, clip]{figures/table-algs-obj.png}
%   \vspace{-5mm}
% \caption{\kbcomm{add caption}}

%   \label{tab:algs-obj}
%   \vspace{-20mm}
% \end{wrapfigure}

While there is a large body of work which studies the properties of LLMs, and especially in-context learning, here we review some of the work which relates most closely with ours.\vspace{-3mm}

\paragraph{Improving in-context learning.} Prompt tuning is a nascent line of work focused on improving the out-of-the-box, in-context task adaptation abilities of LLMs. One line of prompt tuning literature improves performance by carefully designing the natural language specifications of the task (the text prompt) without making any gradient updates to the model~\cite{arora2022ask, wei2022chain}. These methods attempt to boost performance by optimizing the task examples chosen for the prompt~\cite{diao2023active, liu2022makes}, encouraging the models to sequentially reason through tasks~\cite{kojima2022large, wei2022chain, zelikmanstar} and aggregating across multiple prompts~\citep{wang2022self, wang2022rationale}. Unfortunately, prompt-based task adaptation is noisy\citep{lu2022fantastically}, requires manual tuning, and the effectiveness of a prompt is limited by how much information can be fit in the finite context window of the models. In contrast, our work attempts to improve the ICL abilities of LLMs with standard prompting formats alone. Another line of prompt tuning works improves the ICL abilities of models by tuning small amounts of learnable vectors~\citep{li2021prefix,lester2021power, liu-etal-2022-p} for specific tasks. While these methods have been shown to improve ICL performance significantly, they require task-specific finetuning---a key difference to \alg. Another line of work attempts to improve the ``reasoning'' mechanisms of LLMs by modifying decoding strategies. A recent work demonstrates that probabilistic models can be used to impose lexical constraints in text generation~\citep{zhang2023tractable}. Although these methods are task-agnostic, they focus on improving LLM outputs at a token and not task level.\vpsace{-3mm}

\paragraph{Understanding ICL.} 
Recent works seek to understand the in-context learning property of LLMs by exploring the breadth of tasks models can learn in-context, presenting mechanistic interpretations of ICL~\citep{von2022transformers} and performing exploratory analysis of ICL behaviors\citep{wei2023larger}. Existing literature demonstrates that LLMs can learn function classes (e.g., linear regression)~\citep{garg2022can} in-context, and propose that LLMs are performing gradient descent when learning tasks in-context~\citep{von2022transformers}. Another line of work relates ICL ability to structures found in training data~\citep{hahn2023theory, wei2023larger, Shin2022OnTE}. Complementary to these works, we seek to provide insights on the mechanisms of ICL learning, its current deficiencies, and propose a strategy for improving out-of-the-box task-learning.  \vspace{-3mm}


\paragraph{Task-specific LLM Tuning Strategies.} 
%Meta learning literature, adaptors for robustness. 
Task transfer strategies adapt LLMs to a target domain and task. Strategies range from full-finetuning to parameter efficient finetuning (PEFT). Common PEFT tunning strategies include adapters which prepends tunable prompt tensors to the embedded inputs~\citep{houlsby2019parameter, zhang2023llamaadapter} and Low-Rank adaptation (LoRA)~\citep{hu2022lora} which introduces trainable rank decomposition matrices into each layer. While performant, these methods require training models on a task-by-task basis in contrast to \alg. 

%\textbf{\red{Teaching LLMs to reason?}}


% \textbf{Probabilistic reasoning with LLMs.} Calibration of LLMs, Guy paper (and similar works).

==> main/figures.tex <==
\section{Plots for experiments}
\subsection{Plots for Section~\ref{sec:strats}}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-gpt-neo-125m_48.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-pythia-160m-deduped_48.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-bloom-560m_48.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{[ICL-micro] base in context learning vs linear probing on model embeddings}
    \label{fig:icl-micro}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-ft-gpt-neo-125m.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-ft-pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/base-lr-ft-bloom-560m.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{[ICL-micro-2] base in context learning vs linear probing on model embeddings}
    \label{fig:icl-micro2}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_gains_gpt-neo-125m.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_gains_pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_gains_bloom-560m.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{[Micro-1]Representation vs Reasoning gains for fine-tuning.\kbcomm{ add plots for neo and bloom, duplicated right now}}
    \label{fig:rep-reas}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/ft-ag-acc-line-gpt-neo-125m.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/ft-ag-acc-line-pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/ft-ag-acc-line-bloom-560m.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{[Micro-2] Accuracy of fine tuned model on task vs accuracy of fine tuned model on ag news (averaged across 6 datasets}
    \label{fig:agnostic-m2}
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_ft_ag_gpt-neo-125m.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_ft_ag_pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-4/rep_vs_reas_ft_ag_bloom-560m.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{[Micro-3] Loss due to representations vs loss to reasoning abilities}
    \label{fig:agnostic-m3}
\end{figure*}


\subsection{Plots for Section~\ref{sec:fluffy}}

\subsection{Plots for Section~\ref{sec:exp}}
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/scatter_gpt-neo-125m_k_48.png}
        \subcaption{GPT-Neo-125M}
        \vspace{0.2cm}
    \end{subfigure}
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/scatter_pythia-160m-deduped_k_48.png}
        \subcaption{Pythia-160M}
        \vspace{0.2cm}
    \end{subfigure}
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/scatter_bloom-560m_k_48.png}
        \subcaption{Bloom-560M}
    \end{subfigure}
    \caption{[Macro-NLP]Accuracy comparisons for \alg with ICL, Full Fine-tuning, Fine tune last layer, Fine tune adpater head.\kbcomm{add details to caption}}
    \label{fig:macro}
\end{figure*}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/long-context_gpt-neo-125m.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/long-context_pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/plots-section-6/long-context_bloom-560m.png}
        \subcaption{Bloom}
    \end{subfigure}
    \caption{Data scaling plots}
    \label{fig:data-scale}
\end{figure*}




==> main/prob.tex <==
\section{Problem setup}\label{sec:prob}
We introduce the formal problem definition, describe the desiderata for our problem setup, and taxonomize the different task adaptation methods. 

\subsection{Problem description.} 
Given a pre-trained LLM, and limited access to labelled data for a given task. How does one adapt the LLM to this task? Focus will be on binary classification tasks.

\subsection{Evaluation criteria}
We would like the task adaptation strategy to have the following properties:

\paragraph{Task-agnostic.} Would like to have a single model which works well across a variety of different tasks. Foundation model, or pre-trained LLMs, provide a good base for task-agnostic methods since they have general capabilities. Would like the adaptation strategy to preserve this task-agnostic property of these models in the same way as in-context learning methods does.  Interesting because allows the same model to serve different applications. Important since as model sizes increase, gets harder to deploy task-specific ones. Avoids expensive hyper-parameter search. 

\paragraph{Performant.} Would like the task adaptation method to achieve high accuracy on the specified tasks. For the binary classification tasks, we care about prediction accuracy.

\paragraph{Model preservation.} Would like the task adaptation method to change the base model and its representations. Pre-training helps FMs learn general abilities, encoded in their model weights, which can be independently evaluated. Would like these general abilities and the associated representations to persist for the specific task.

\subsection{Task adaptation strategies}
We can broadly taxonomize the different task adaptation strategies as in-context learning, fine tuning the model, and training task-specific adapter heads. We describe where they stand with respect to the evaluation criteria described above. (see figure \kbcomm{insert a figure here}).

\paragraph{In-context learning.} In-context learning learning allows to adapt the model without updating any model parameters, by simply providing a few demonstrations of the task within the prompt. The predicted label is obtained by looking at the next word generated by the LLM. ICL is completely task-agnostic since the same model can be used across tasks, and preserves the model entirely since no weights are updated at inference time. However, its performance is usually not at par when compared with task-specific methods (see figure) and the number of examples one can use with ICL is often bottlenecked by the context length of the model. 

\paragraph{Fine tuning.} These methods update the model parameters to adapt it to the task. Fine tuning methods typically take multiple passes over the labelled set and use the gradients with respect to the predicted loss to perform the updates. Depending on which layers of the model are updated, there is a whole hierarchy of fine tuning methods. Full fine tuning (Full FT) updates all the parameters of the model, last layer fine tuning (FT-last layer) involves updating the final layer + the language model head, and finally one can also just update the language model head (FT-LM head). This class of methods are not task agnostic, changes the underlying model significantly, but usually have very good performance since the model is adapted to the task. 

\paragraph{Adapter heads.} This class of methods uses the frozen model backbone along with an additional set of updatable parameters (typically a one layer FCN) to adapt the underlying model to the specified task. In contrast to fine tuning, which performs updates to the base model, Adapter heads keep the base model frozen and only updates the additional parameters. These methods are also task-specific like the fine tuning methods but preserve the underlying base model. We show in our experimental evaluations (see Section~\ref{sec:exp} that these methods also have performance comparable to the fine tuning methods. 

==> main/rep-reas.tex <==
\section{Understanding performance via Representation-Reasoning decomposition}\label{sec:rep-reas}
In this section, we consider the hypothesis why the task-agnostic ICL method has lower quality, in terms of accuracy, when compared with task-specific fine tuning and adapter heads. Key insight is that this performance can be explained via a representation-reasoning decomposition, that is, the while the model has sufficient information in the underlying representations, it lacks in the reasoning abilities to make the correct inference. We first describe the experimental setup and then analyse the different methods for this.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/rep-reas/rep_vs_reas_gains_pythia-160m-deduped.png}
        \subcaption{GPT-Neo}
    \end{subfigure}
     \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/rep-reas/rep_vs_reas_gains_pythia-160m-deduped.png}
        \subcaption{Pythia}
    \end{subfigure}
     \begin{subfigure}[b]{0.28\textwidth}
        \centering
        \includegraphics[width=\textwidth]{plots/rep-reas/rep_vs_reas_gains_pythia-160m-deduped.png}
        \subcaption{Bloom}
    \end{subfigure}
    \label{fig:rep-reas}
    \caption{Representation vs Reasoning gains for fine-tuning.\kbcomm{ add plots for neo and bloom, duplicated right now}}
\end{figure*}

\subsection{Main hypotheses}
\begin{enumerate}
    \item Models representations have enough information to perform the task in-context, but it lacks the reasoning abilities to make the correct inference.
    \item Fine-tuning changes both reps and reasoning, reasoning is more instrumental in aligning model for task. Lowers task agnosticity.
    \item Adapter based methods only affect reasoning. Leads to gains on the specific task. Performance is lower when try to trasnfer to other tasks.
\end{enumerate}

\subsection{Experimental setup}
\paragraph{In-context learning.} Describe the last layer representations, logistic regression on representations as a baseline for reasoning abilities. 

\paragraph{Fine-tuning.} For fine tuning, we will compute two scores: representation gains: fine-tune+LR-solver - base+LR-solver and reasoning gains: Base ICL - fine-tune ICL as proxies. Justify why these are good proxies for measure these gains and finally how we will use them to get the final conclusions. 
To get an understanding of the task-agnostic power of these methods, will compute the two scores again, 
representation loss: train LR solver on fine tuned model vs train LR solver on base model
reasoning loss: perform ICL on fine tuned model vs perform icl on base model

\paragraph{Adapter heads.} For the adapter heads, the representations are not affected, only the final layer is modified. 
Representation loss = 0
reasoning loss: accuracy with head on ag-news vs accuracy with head on actual dataset.

\subsection{Analysis of various task-adaptation methods}
\subsubsection{In-context learning}
\kbcomm{Insert plot:Base ICL accuracy vs. LR solver accuracy (scatter plot)}\\
Main takeaway:  ICL has enough representation ability, lacks in inference ability.

\subsubsection{Fine tuning methods}
\kbcomm{Insert plot: Representation gains vs reasoning gains (scatter plot)}\\
Main takeaway: Fine tuning works better than ICL because reasoning (or representation gains) are much higher.

\kbcomm{Insert plot: task Agnosticity, scatter plot - accuracy (ft-data) vs accuracy (ft-ag-news)}\\
Main takeaway: see an accuracy loss when use fine tuned models on different datasets -- not task agnostic.

\kbcomm{Insert plot: task agnosticity, scatter plot, representation loss vs reasoning loss}\\
Main takeaway: loss is explained by overfitting of one of these patterns to the data. 

\subsubsection{Adapter heads}
\kbcomm{Insert plot: Base model vs adapter heads (scatter plot)}\\
Main takeaway: Adapter heads improve reasoning ability for the specific task they are trained on.

\kbcomm{Insert plot:  task Agnosticity, scatter plot - accuracy (ft-data) vs accuracy (ft-ag-news)}\\
Main takeaway: Adapters also overfit to the current task distributions.
